Retina-Inspired Object Motion Segmentation for Event-Cameras

Event-cameras have emerged as a revolutionary technology with a high temporal resolution that far surpasses standard active pixel cameras. This technology draws biological inspiration from photoreceptors and the initial retinal synapse. This research showcases the potential of additional retinal functionalities to extract visual features. We provide a domain-agnostic and efficient algorithm for ego-motion compensation based on Object Motion Sensitivity (OMS), one of the multiple features computed within the mammalian retina. We develop a method based on experimental neuroscience that translates OMS' biological circuitry to a low-overhead algorithm to suppress camera motion bypassing the need for deep networks and learning. Our system processes event data from dynamic scenes to perform pixel-wise object motion segmentation using a real and synthetic dataset. This paper introduces a bio-inspired computer vision method that dramatically reduces the number of parameters by $\text{10}^\text{3}$ to $\text{10}^\text{6}$ orders of magnitude compared to previous approaches. Our work paves the way for robust, high-speed, and low-bandwidth decision-making for in-sensor computations.

==> src/algo.tex <==
\noindent
We investigate a static implementation of Object Motion Sensitivity (OMS) from experimental neuroscience~\cite{schwartz2021object}. The visual pathways of many biological organisms have evolved the OMS circuit to suppress stimuli created by ego-motion from body and eye movements. As shown in Figure~\ref{fig:oms_circuit}, this circuit is comprised of bipolar (BC), amacrine (AC), and ganglion cell (RGC) layers, which work together to distinguish between stimuli created by global and local motion.  
Neuroscience foundations define the role these cells play in OMS~\cite{schwartz2021object}. BCs adapt rapidly to changes in luminance. Within the retina, dedicated BCs exist to transmit information about both light increases and decreases. ACs integrate contrast signals from a global area (surround) and subtract them from the local area (center). This computation acts like a spatial filter that detects changes in movement between global and local areas. Subsequently, the RGCs respond to local motion in the receptive field ‘center’ or differential motion of the 'center' and 'surround' regions of the receptive field while remaining silent for global motion. Taking inspiration from these mechanisms, Algorithm~\ref{oms_neuro} proposes an approximation of these retinal computations behind OMS.

\begin{algorithm}[h]    
\caption{OMS - Neuroscience}\label{oms_neuro}
\begin{algorithmic}[1]
\Require {radius $r_1$ $<$ radius $r_2$}
\Procedure{OMS}{$dvsFrames$, $r_1$, $r_2$, $s_s$, $\alpha$}
\State $s_c\gets s_s + r_2 - r_1$
\State $center\gets gaussianKernel(r_1)$
\State $surr \gets gaussianKernel(r_2)$

\For{$i$ in $len(dvsFrames)$}{}
    \State $frames \gets dvsFrames[i]$
    \State $fil\_c \gets applyKernel(center, frames, s_c)$
    \State $fil\_s \gets applyKernel(surr, frames, s_s)$
    \State $events \gets fil\_c - fil\_s$
    \State $OMS[i] \gets events > \alpha$
\EndFor
\State \textbf{return} $OMS$
\EndProcedure
\end{algorithmic}
\end{algorithm}

\noindent
This algorithm begins with the definition of a series of parameters described below. 
\begin{itemize}
    \item \textbf{Input frames ($dvsFrames$)} store photoreceptor activations within BCs. Our practical approach projects the events into a frame by compressing the time and polarity domain. This input provides the binary values mimicking BC output. 
    \item \textbf{Center ($center$) and surround kernels ($surr$)} represent two circular Gaussian kernels of a chosen radius ($r_1$ and $r_2$), whose discrete values are sampled from a normalized Gaussian distribution. 
    \item \textbf{Radius ($r_1$ and $r_2$)} represent the radius values that define the discrete circles in the filters' matrices.
    \item \textbf{Strides of the center ($s_c$) and surround ($s_s$) kernels}.
    \item \textbf{Threshold} ($\alpha$) decides whether motion is detected for a pixel.
\end{itemize}

%\begin{figure}[t]
 %   \centering
    %\includegraphics[width=0.3575\textwidth]{figures/kernel_visualization.png}
    %\caption{A visualization of the Gaussian kernel for the algorithmic implementation of Object Motion Sensitivity.}
    %\label{fig:kernel-vis}
%\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/oms_circuit.png}
    \caption{Retinal object motion sensitivity circuit}
    \label{fig:oms_circuit}
\end{figure}
The DVS frames represent the response to photoreceptor activation by BCs, and our algorithm performs the computations of the AC and RGC layers. The OMS algorithm consists of two circular averaging filters, also known as disk filters~\cite{MATLAB}. These kernels are matrices containing a discrete feathered circle of a chosen radius whose values sum to one. The values in the center of the matrix are larger and therefore carry more significance.
The smaller of these kernels is the center kernel, which represents an RGC and the excitatory BC cluster to which it is connected, see Figure~\ref{fig:oms_circuit}. We set the radius $r_1 = 2$ since it lowers the likelihood that a single cell cluster will cover an entire object. 

The surround kernel serves as the AC and its corresponding BC cluster, which is designed to inhibit the RGCs' response if global motion is perceived, see Figure~\ref{fig:oms_circuit}. For this kernel, a $r_2$ of $4$ was chosen to cover a sufficiently wide region of each frame without significantly reducing the weight around the edges. The radius values were used for both datasets, showcasing the strong generalization of this algorithm.

In the algorithm's execution, the kernels convolve over the frames by centering themselves over each pixel and storing the resultant value in the position of said pixel. This value is the mean contrast of the region covered by the disk filter. The surround kernel convolves over the frame with a stride of $s_s = 1$. However, to keep the center kernel centered over the surround kernel, the stride of the center kernel is dynamically calculated based on the stride of the surround kernel with the difference in kernel radii.

Finally, to simulate inhibition, the mean contrast values from the surround kernel are subtracted from those of the center kernel, see inhibitory and excitatory synapses in Figure \ref{fig:oms_circuit}. If the resultant values are larger than a threshold ($\alpha$), then a binary spike is stored in the OMS frame. 
The threshold value was found empirically and set to $\alpha = 0.96$ for the EV-IMO dataset \cite{mitrokhin2020evimo}, see Figure \ref{fig:threshold}. The selected value offered a balance between preserving the object structure and suppressing background interference. In contrast, we selected a threshold of $\alpha = 0.5$ for MOD \cite{MOD} because of the reduced spike density.

\begin{figure}
\centering
    \includegraphics[width=0.375\textwidth]{figures/threshold.png}
\caption{Frames from OMS for different threshold ($\alpha$) values. Frames taken from EV-IMO \cite{mitrokhin2020evimo} dataset.}
\label{fig:threshold}
\end{figure}



